Coalition Formation and Combinatorial Auctions; Applications to Self-organization and Self-management in Utility Computing

In this paper we propose a two-stage protocol for resource management in a hierarchically organized cloud. The first stage exploits spatial locality for the formation of coalitions of supply agents; the second stage, a combinatorial auction, is based on a modified proxy-based clock algorithm and has two phases, a clock phase and a proxy phase. The clock phase supports price discovery; in the second phase a proxy conducts multiple rounds of a combinatorial auction for the package of services requested by each client. The protocol strikes a balance between low-cost services for cloud clients and a decent profit for the service providers. We also report the results of an empirical investigation of the combinatorial auction stage of the protocol.

==> SelfManagement.tex <==
%****************************************************************
\section{Self-organization}
\label{SelfOrganization}
\medskip
%****************************************************************

\smallskip







==> SubCoalitionFormation.tex <==
%****************************************************************
\section{Sub-coalition Formation and Consensus Algorithms}
\label{SubCoalitionFormation}
%****************************************************************

In a clustered organization the {\it cluster leader} manages the formation of the sub-coalition offering services in each auction. A {\it sub-coalition} consists of  servers willing to provide a set of services. The members of a sub-coalition are located in ``proximity'' to one another and thus benefit from lower latency and higher bandwidth. A {\it consensus algorithm} allows the members of a sub-coalition to elect a leader who can negotiate on their behalf; they also agree on the price for the services and resources its members are willing to offer during the auction. We now justify the need for sub-coalitions, present a consensus algorithm, and introduce the  agreement regarding the price for services provided by a sub-coalition.

\smallskip

{\bf Why form sub-coalitions?}  Sub-coalitions support aggregation of resources and of services. Resource  aggregation is necessary because a single platform may not be able to provide the resources demanded by a cloud client. Service aggregation is necessary to reduce the number of agents involved in an auction thus,  the time and space requirements of the auctioning algorithms.


A third motivation is to reduce the computing and communication costs. This requires resource management mechanisms that exploit the organization of  the cloud infrastructure. Spatial and temporal locality are critical requirements for the functionality of the protocol being proposed here. 

{\it Spatial locality} means that an auction should favor packages which involve servers in the same sub-coalition; spatial locality reduces the communication costs. {\it Temporal locality} means that an auction should favor reservations consisting of a run of consecutive slots. This reduces the overhead involved in saving partial results and then reloading them at a later time. The auctions provide incentives for packages that use services offered by one sub-coalition over a run of consecutive slots.




\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=12cm]{figures/Paxos.eps}
\end{center}
\caption{The flow of messages to reach consensus. The message types: \underline{1. Prepare} -- the leader chooses a proposal with proposal number $pn=j$; \underline{2. Promise}  -- an acceptor promises to accept the proposal only if it has not responded to a proposal with $pn> j$; B does not respond; \underline{3. Accept request} -- the leader chooses the value $v$ of the highest proposal number from all acceptors who have sent a promise and sends it to all of them; \underline{4. Accept} -- an acceptor accepts a proposal with $pn=j$ only if it has not promised to accept a proposal with $pn >j$; it stores the accepted value in persistent memory. \underline{5. Proposal accept} -- the leader accepts a proposal if the quorum of acceptors send an accept message for the proposal with $pn=j$; A accepts, while C does not accept.}
\label{PaxosFig}
\end{figure*}

{\bf A consensus algorithm.} A cluster leader uses a Paxos-type algorithm \cite{Lamport98, Lamport01} to determine the price range the sub-coalition can agree on. The {\it basic Paxos} considers several types of entities: (a) {\it client,} an agent that issues a request and waits for a response; (b) {\it proposer,} an agent with the mission to advocate a request from a client, convince the acceptors to agree on the value proposed by a client, and to act as a coordinator moving  the protocol forward in case of conflicts; (c) {\it acceptor}, an agent acting as the fault-tolerant ``memory'' of the protocol; (d) {\it learner,} an agent acting as the replication factor of the protocol and taking action once a request has been agreed upon; and finally (e) the {\it leader,} a distinguished proposer. A {\it quorum} is a subset of all acceptors.

The flow of messages can be described as follows \cite{Lamport01}: ``clients send messages to a leader; during normal operations the leader receives the client's command, assigns it a new command number $i$, and then begins the $i$-th instance of the consensus algorithm by sending messages to a set of acceptor processes.'' A proposal consists of a pair, $(pn, v)$, with $pn$  a unique proposal number and $v$ a proposed value; multiple proposals may propose the same value $v$. A value $v$ is chosen if a simple majority of  acceptors have accepted it.  We need to guarantee that at most one value can be chosen, otherwise there is no consensus.  The phases of the algorithm are:


\smallskip

\begin{enumerate}
\item
{\it Proposal preparation:} a proposer (the leader) sends a proposal $(pn=j,v)$. The proposer chooses a proposal number $pn=j$ and sends a {\it prepare message} to a majority of acceptors requesting: (a)
that a proposal with $pn < j$ should not be accepted; (b) the $pn < j$ of the highest number proposal already accepted by each acceptor.
\item
{\it Proposal promise:} An acceptor must remember the proposal number of the highest proposal number it has ever accepted as well as the highest proposal number it has ever responded to. The acceptor  can accept a proposal with $pn=j$ if and only if it has not responded to a prepare request with $pn > j$; if it has already replied to a prepare request for a proposal with $pn > j$ then it should not reply. Since they are indistinguishable, lost messages are treated as an acceptor that chooses not to respond.
\item
{\it Accept request:} if the majority of acceptors respond, then the proposer chooses the value $v$ of the proposal as follows: (a) the value $v$ of the highest proposal number selected from all the responses; (b) an arbitrary value if no proposal was issued by any of the proposers.
The proposer sends an {\it accept request} message to a quorum of acceptors including $(pn=j,v)$.

\item
{\it Accept:} If an acceptor receives an {\it accept message} for a proposal with the proposal number $pn=j$ it must accept it, if and only if, it has not already promised to consider proposals with a $pn > j$. If it accepts the proposal it should register the value $v$ and send an {\it accept} message to the proposer and to every learner; if it does not accept the proposal it should ignore the request.
\end{enumerate}


Figure \ref{PaxosFig}\cite{Marinescu13a} illustrates the flow of messages for the consensus protocol. By merging the three roles, proposer, acceptor, and learner, the protocol ``collapses'' into an efficient client-master-replica style protocol.


\medskip

{\bf Reaching agreement regarding the price for services.} In our case, the suppliers, the autonomous servers able and willing to respond to a request for service reservations, play the role of both clients and acceptors. They propose  a price per unit of service and, eventually, agree on one of the proposals. The cluster-leader coordinates the consensus procedure.

Now we provide more detail on the sub-coalition formation process.  A supply agent, $\mathbb{C}_{k,i}$, wishing to join sub-coalition $\mathbb{C}_{k}$ provides the leader with two parameters, $q_{k,i}$ the quantity and $c_{k,i}$ the supplier's internal cost per unit of service. We assume that the members of sub-coalition $\mathbb{C}_{k}$, $\{ \mathbb{C}_{k,1}, \mathbb{C}_{k,2},\ldots, \mathbb{C}_{k,{n_{k}}} \}$, are listed in the order of their internal costs per unit of service

\begin{equation}
c_{k,1} \le c_{k,2} \ldots \le c_{k,{n_{k-1}}} \le c_{k,{n_{k}}}
\end{equation}
The price for the unit of service the coalition chooses should satisfy the condition:


\begin{equation}
\label{PriceRangeEq}
p_{k} \ge c_{k,{n_{k}}}
\end{equation}


Then the {\it value}, $\mathcal{V}_{k}$, of sub-coalition $\mathbb{C}_{k}$   is defined as  the difference between  the price of the package auctioned by $\mathbb{C}_{k}$ and the internal costs of the individual members

\begin{equation}
\mathcal{V}_{k} = p_{k} \sum_{i=1}^{n_{k}} q_{k,i} - \sum_{i=1}^{n_{k}} q_{k,i} c_{k,i}
\end{equation}
The {\it value per unit of service} of sub-coalition $\mathbb{C}_{k}$ and the reward or the individual payoff of the agent $\mathbb{C}_{k,i}$ are, respectively,

\begin{equation}
v_{k} =  { \mathcal{V}_{k} \over {\sum_{i=1}^{n_{k}} q_{k,i}  }}
~~\text{and}~~
r_{k,i} = q_{k,i} ( p_{k} - c_{k,i})
\end{equation}
A {\it payoff division} is a vector reflecting the financial gains of individual members of $\mathbb{C}_{k}$

\begin{equation}
\mathcal{R}_{k} = \{ r_{k,1}, r_{k,2}, \ldots, r_{k,n_{k}} \}
\end{equation}
The {\it core} of a sub-coalition is the collection of all payoff divisions such that
$r_{k,i} > 0 ~~\forall i \in \{1, n_{k} \}$.

The sub-coalition $\mathbb{C}_{k}$ is said to be {\it stable in the core} if the
corresponding payoff vector $\mathcal{R}_{k}$ is in the core. The condition given by Equation \ref{PriceRangeEq} guaranties stability in the core. The leader communicates $c_{k,{n_{k}}}$ to the members of the sub-coalition and requests proposals for the sub-coalition  target value. The agreed target value determines the price for the particular service. The total number of messages exchanged to establish the consensus in a sub-coalition  with $n_{k}$ members, including the leader, is $N_{k}^{msg} \le 8 \times (n_{k} - 1)$.

